SPI-Optimizer: an integral-Separated PI Controller for Stochastic Optimization

To overcome the oscillation problem in the classical momentum-based optimizer, recent work associates it with the proportional-integral (PI) controller, and artificially adds D term producing a PID controller. It suppresses oscillation with the sacrifice of introducing extra hyper-parameter. In this paper, we start by analyzing: why momentum-based method oscillates about the optimal point? and answering that: the fluctuation problem relates to the lag effect of integral (I) term. Inspired by the conditional integration idea in classical control society, we propose SPI-Optimizer, an integral-Separated PI controller based optimizer WITHOUT introducing extra hyperparameter. It separates momentum term adaptively when the inconsistency of current and historical gradient direction occurs. Extensive experiments demonstrate that SPIOptimizer generalizes well on popular network architectures to eliminate the oscillation, and owns competitive performance with faster convergence speed (up to 40% epochs reduction ratio ) and more accurate classification result on MNIST, CIFAR10, and CIFAR100 (up to 27.5% error reduction ratio) than the state-of-the-art methods.

==> sections/figures/CI.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/CI} % don't need to specify .png or .jpg
\caption{ci}
\label{/fig:ci}
\end{figure}

==> sections/figures/block.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/kuangtu} % don't need to specify .png or .jpg
\caption{PI Controller block diagram}
\label{/fig:PI Controller block diagram}
\end{figure}


==> sections/figures/c100_alexnet.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet} % don't need to specify .png or .jpg

\newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c100_alexnetl}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c100_alexnet}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}

\caption{Comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-100 dataset using AlexNet as the architecture for 50 epochs.Left: the curves of validation loss.Right: the curves of validation accuracy   }
\label{/fig:c100_alexnet}
\end{figure}

==> sections/figures/c100_alexnet2.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet2} % don't need to specify .png or .jpg
\caption{图17是学习率为0.05(50个epoch,我按照你之前说的,其实只放了38个epoch,因为后面开始过拟合效果不好了,但只有这张图是38epoch,其他图都是50epoch,我不清楚不统一会不会不好).Comparison of SPI and popular optimization methods(MOM, SGD, NAG) on the CIFAR-100 dataset using AlexNet as the architecture for 50 epochs.Top row: the curves of training loss and validation loss.Bottom row: the curves of training accuracy and validation accuracy  }
\label{/fig:c100_alexnet2}
\end{figure}

==> sections/figures/c100_alexnet_jf.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet_jf} % don't need to specify .png or .jpg
\caption{Comparison of SPI-Optimizer and CI with 7 different thresholds on the CIFAR-100 dataset using AlexNet as the architecture for 50 epoches }
\label{/fig:c100_jf}
\end{figure}

==> sections/figures/c100_alexnet_lr.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet_lr} % don't need to specify .png or .jpg
\caption{With stable learning rate(No attenuation),comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-100 dataset using AlexNet as the architecture for 200 epochs.}
\label{/fig:c100_alexnet_lr}
\end{figure}

==> sections/figures/c100_difflr.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_difflr} % don't need to specify .png or .jpg
\caption{Performance comparison of SPI-Optimizer with different learning rate on CIFAR-100 using AlexNet}
\label{/fig:C100_difflr}
\end{figure}

==> sections/figures/c100_wrn.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100wrn} % don't need to specify .png or .jpg
\caption{Train on the CIFAR-100 dataset using Wide-ResNet \cite{zagoruyko2016wide} for 200 epochs.}
\label{/fig:c100_wrn}
\end{figure}




==> sections/figures/c10_alexnet.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_alexnet} % don't need to specify .png or .jpg
 \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c10_alexnetl}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c10_alexnet}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}
\caption{comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-10 dataset using AlexNet as the architecture for 50 epochs.Left: the curves of validation loss.Right: the curves of validation accuracy }
\label{/fig:c10_alexnet}
\end{figure}

==> sections/figures/c10_alexnet_jf.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_alexnet_jf} % don't need to specify .png or .jpg
\caption{Comparison of SPI-Optimizer and CI with 7 different thresholds on the CIFAR-10 dataset using AlexNet as the architecture for 50 epoches }
\label{/fig:c10_jf}
\end{figure}

==> sections/figures/c10_alexnet_lr.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_alexnet_lr} % don't need to specify .png or .jpg
\caption{With stable learning rate(No attenuation), comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-10 dataset using AlexNet as the architecture for 200 epochs.}
\label{/fig:c10_alexnet_lr}
\end{figure}

==> sections/figures/c10_difflr.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_difflr} % don't need to specify .png or .jpg
\caption{Performance comparison of SPI-Optimizer with different learning rate on CIFAR-10 using AlexNet}
\label{/fig:C10_difflr}
\end{figure}

==> sections/figures/c10_wrn.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_wrn} % don't need to specify .png or .jpg

 \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c10_wrnl}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c10_wrn}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}

\caption{Comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-10 dataset using Wide-ResNet\cite{zagoruyko2016wide} as the architecture for 200 epochs.Left: the curves of validation loss.Right: the curves of validation accuracy   }
\label{/fig:c10_wrn}
\end{figure}

==> sections/figures/e23alexnet.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_alexnet} % don't need to specify .png or .jpg
 \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/e2_alexnetc10}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/e3_alexnetc100}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}
\caption{comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-10 dataset using AlexNet as the architecture for 50 epochs.Left: the curves of validation loss.Right: the curves of validation accuracy }
\label{/fig:c10_alexnet}
\end{figure}

==> sections/figures/e45resnet.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_alexnet} % don't need to specify .png or .jpg
 \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/e4_resnet56c10}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/e5_resnet56c100}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}
\caption{comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-10 dataset using AlexNet as the architecture for 50 epochs.Left: the curves of validation loss.Right: the curves of validation accuracy }
\label{/fig:c10_alexnet}
\end{figure}

==> sections/figures/e89wrn.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c10_alexnet} % don't need to specify .png or .jpg
 \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/e8_wrnc10}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/e9_wrnc100}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}
\caption{comparison of SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) on the CIFAR-10 dataset using AlexNet as the architecture for 50 epochs.Left: the curves of validation loss.Right: the curves of validation accuracy }
\label{/fig:c10_alexnet}
\end{figure}

==> sections/figures/f11_lag.tex <==
\begin{figure}[ht!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet} % don't need to specify .png or .jpg

\newcommand{\colw}{0.48}
    \newcommand{\figw}{0.98} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_00}}}
        \captionsetup{labelformat=empty}
        \caption{a: MOM's trajectory}
        \label{/fig:mom_lag_a}
    \end{subfigure}
    
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f11overmom}}}
        \captionsetup{labelformat=empty}
        \caption{b: MOM}
        \label{/fig:mom_lag_mom}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f11oversgd}}}
        \captionsetup{labelformat=empty}
        \caption{c: GD}
        \label{/fig:mom_lag_gd}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f11overnag}}}
        \captionsetup{labelformat=empty}
        \caption{d: NAG}
        \label{/fig:mom_lag_nag}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f11overm99}}}
        \captionsetup{labelformat=empty}
        \caption{e: SPI}
        \label{/fig:mom_lag_isp}
    \end{subfigure}
\caption{(a): convergence path of MOM on a 2D toy convex function $f_1(\theta)$ with colored segments representing each weight update. (b-e): horizontal residual w.r.t. the optimal point versus time. Two components for the weight update are the current gradient (red arrow) and the momentum (green arrow), which can be interpreted as two forces dragging the blue curve.}
\label{/fig:mom_lag}
\end{figure}

==> sections/figures/f3_lag.tex <==
\begin{figure}[ht!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet} % don't need to specify .png or .jpg

\newcommand{\colw}{0.48}
    \newcommand{\figw}{0.98} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_0_-2_1}}}
        \captionsetup{labelformat=empty}
        \caption{a: MOM's trajectory}
        \label{/fig:mom_lag_a}
    \end{subfigure}
    
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f3overmom}}}
        \captionsetup{labelformat=empty}
        \caption{b: MOM}
        \label{/fig:mom_lag_mom}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f3oversgd}}}
        \captionsetup{labelformat=empty}
        \caption{c: GD}
        \label{/fig:mom_lag_gd}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f3overnag}}}
        \captionsetup{labelformat=empty}
        \caption{d: NAG}
        \label{/fig:mom_lag_nag}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f3overm99}}}
        \captionsetup{labelformat=empty}
        \caption{e: SPI}
        \label{/fig:mom_lag_isp}
    \end{subfigure}
\caption{(a): convergence path of MOM on a 2D toy convex function $f_1(\theta)$ with colored segments representing each weight update. (b-e): horizontal residual w.r.t. the optimal point versus time. Two components for the weight update are the current gradient (red arrow) and the momentum (green arrow), which can be interpreted as two forces dragging the blue curve.}
\label{/fig:mom_lag}
\end{figure}

==> sections/figures/f5_lag.tex <==
\begin{figure}[ht!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet} % don't need to specify .png or .jpg

\newcommand{\colw}{0.48}
    \newcommand{\figw}{0.98} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_00}}}
        \captionsetup{labelformat=empty}
        \caption{a: MOM's trajectory}
        \label{/fig:mom_lag_a}
    \end{subfigure}
    
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f5overmom}}}
        \captionsetup{labelformat=empty}
        \caption{b: MOM}
        \label{/fig:mom_lag_mom}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f5oversgd}}}
        \captionsetup{labelformat=empty}
        \caption{c: GD}
        \label{/fig:mom_lag_gd}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f5overnag}}}
        \captionsetup{labelformat=empty}
        \caption{d: NAG}
        \label{/fig:mom_lag_nag}
    \end{subfigure}
        ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/f5overm99}}}
        \captionsetup{labelformat=empty}
        \caption{e: SPI}
        \label{/fig:mom_lag_isp}
    \end{subfigure}
\caption{(a): convergence path of MOM on a 2D toy convex function $f_1(\theta)$ with colored segments representing each weight update. (b-e): horizontal residual w.r.t. the optimal point versus time. Two components for the weight update are the current gradient (red arrow) and the momentum (green arrow), which can be interpreted as two forces dragging the blue curve.}
\label{/fig:mom_lag}
\end{figure}

==> sections/figures/function_loss_curve01.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/function_loss_curve1} % don't need to specify .png or .jpg
    \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/function_loss_curve1}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/function_loss_curve2}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}
\caption{Curves of loss $\log (\norm{e})$ v.s. NO. of iterations. SPI-Optimizer performs the best among the methods GD, MOM, NAG, and CI with different $\beta$ on both the functions $f1(x,y)$ and $f2(x,y)$}
\label{fig:function_loss_curve1}
\end{figure}



==> sections/figures/function_loss_curve03.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/function_loss_curve3} % don't need to specify .png or .jpg
\caption{Loss curve of SPI, CI with different T (threshold), and popular optimization methods (MOM, SGD, NAG) on the Rosenbrock function:$f(x,y)=(1-x)^2+100(y-x^2)(y-x^2)$.}
\label{fig:function_loss_curve3}
\end{figure}

==> sections/figures/function_loss_curvef02.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/function_loss_curve2} % don't need to specify .png or .jpg
\caption{loss curves (l2log) of SPI, CI with different T(threshold) and popular optimization methods (MOM, SGD, NAG) on the function$ f(x,y)=x^2+50y^2$}
\label{fig:function_loss_curve2}
\end{figure}

==> sections/figures/hyperparameter.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/c100_alexnet} % don't need to specify .png or .jpg

\newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c10_alexnet_jf}}}
        \captionsetup{labelformat=empty}
        \caption{c10_alexnet,CI-$\beta$ }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/c100_yz}}}
        \captionsetup{labelformat=empty}
        \caption{c100_alexnet,CI-$\beta$ }
    \end{subfigure}

\caption{hyperparameter}
\label{/fig:hyperparameter}
\end{figure}

==> sections/figures/mnist_cnn.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/mnist_cnn} % don't need to specify .png or .jpg

 \newcommand{\colw}{0.48}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/mnistl}}}
        \captionsetup{labelformat=empty}
        %\caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/mnist_cnn}}}
        \captionsetup{labelformat=empty}
        %\caption{b}
    \end{subfigure}


\caption{Comparison of SPI-Optimizer and popular optimization methods (MOM, SGD, NAG) on the MNIST dataset using CNN as the architecture for 20 epochs. Left: the curves of validation loss. Right: the curves of validation accuracy.}
\label{/fig:mnist_cnn}
\end{figure}


%\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/function_loss_curve1} % don't need to specify .png or .jpg




==> sections/figures/mnist_difflr.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/mnist_difflr} % don't need to specify .png or .jpg
\caption{我觉得这个可以删掉,因为后文的表格1已经具有了说明学习率范围的功能,放着给你看看:不同学习率曲线(非平均run5的曲线,就取了个相同seed的不同学习率,意思意思表示)}
\label{/fig:mnist_difflr}
\end{figure}

==> sections/figures/mnist_fnn.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/mnist_fnn} % don't need to specify .png or .jpg
\caption{comparison of 4 popular methods on the MNIST dataset using FNN as the architecture for 20 epochs.Top row: the curves of training loss and validation loss.Bottom row: the curves of training accuracy and validation accuracy  }
\label{/fig:mnist_fnn}
\end{figure}

==> sections/figures/mnist_jf.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/mnist_jf} % don't need to specify .png or .jpg
\caption{Comparison of SPI-Optimizer and CI with 7 different thresholds on the MNIST dataset using CNN as the architecture for 20 epoches.}
\label{/fig:mnistjf}
\end{figure}

==> sections/figures/trajectory_Goldstein_Price_function.tex <==

\begin{figure}[htbp]
    \centering
    % \newcommand{\colw}{0.48}
    % \newcommand{\figw}{1} % can bigger than 1
    \newcommand{\colw}{0.305}
    \newcommand{\figw}{1.0} % can bigger than 1
    \begin{subfigure}[b]{0.8\linewidth}
        \includegraphics[width=1.0\textwidth,clip]{{{sections/figures/figure_files/function_loss_curve11}}}
        \captionsetup{labelformat=empty}
        %\caption{\textbf{SPI}}
    \end{subfigure}%
    
     % leave a blank line to change row     
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_03}}}
        \captionsetup{labelformat=empty}
         \caption{\textbf{SPI}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_01}}}
        \captionsetup{labelformat=empty}
        \caption{GD}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_00}}}
        \captionsetup{labelformat=empty}
        \caption{MOM}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_02}}}
        \captionsetup{labelformat=empty}
        \caption{NAG}
    \end{subfigure}
    ~ 
    % \begin{subfigure}[b]{\colw\linewidth}
    %     \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_04}}}
    %     \captionsetup{labelformat=empty}
    %     \caption{CI-β=0.1}
    % \end{subfigure}
    % ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_05}}}
        \captionsetup{labelformat=empty}
        \caption{CI-β=1}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_06}}}
        \captionsetup{labelformat=empty}
        \caption{CI-β=10}
    \end{subfigure}
    % ~ 
    % \begin{subfigure}[b]{\colw\linewidth}
    %     \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_07}}}
    %     \captionsetup{labelformat=empty}
    %     \caption{CI-β=100}
    % \end{subfigure}
    % ~ 
    % \begin{subfigure}[b]{\colw\linewidth}
    %     \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/11_-4_4.5_08}}}
    %     \captionsetup{labelformat=empty}
    %     \caption{CI-β=1000}
    % \end{subfigure}
%    \caption{comparison of 4 popular methods on the MNIST dataset using CNN as the architecture for 20 epochs.Top row: the curves of training loss and validation loss.Bottom row: the curves of training accuracy and validation accuracy }
    \caption{Convergence comparison within 100 iterations among our SPI-Optimizer, Momentum (MOM) \cite{rumelhart1986learning}, Gradient Descent (GD) \cite{cauchy1847methode}, Nesterov Accelerated Gradient (NAG)  \cite{nesterov1983method} and conditional integral (CI-$\beta$) on the quadratic function $f_4(\theta)$.

        } 
   \label{fig:gold}
\end{figure}

==> sections/figures/trajectory_cos.tex <==

\begin{figure}[t]
    \centering
    \newcommand{\colw}{0.305}
    \newcommand{\figw}{1.0} % can bigger than 1
    \begin{subfigure}[b]{0.8\linewidth}
        \includegraphics[width=1.0\textwidth,clip]{{{sections/figures/figure_files/function_loss_curve3}}}
        \captionsetup{labelformat=empty}
        %\caption{\textbf{SPI}}
    \end{subfigure}%
    
    % leave a blank line to change row       
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_3_-2_1}}}
        \captionsetup{labelformat=empty}
         \caption{\textbf{SPI}}
    \end{subfigure}%
    ~
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_1_-2_1}}}
        \captionsetup{labelformat=empty}
        \caption{GD}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_0_-2_1}}}
        \captionsetup{labelformat=empty}
        \caption{MOM}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_2_-2_1}}}
        \captionsetup{labelformat=empty}
        \caption{NAG}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_5_-2_1}}}
        \captionsetup{labelformat=empty}
        \caption{CI-$\beta=1$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_6_-2_1}}}
        \captionsetup{labelformat=empty}
        \caption{CI-$\beta=10$}
    \end{subfigure}
%    \caption{comparison of 4 popular methods on the MNIST dataset using CNN as the architecture for 20 epochs.Top row: the curves of training loss and validation loss.Bottom row: the curves of training accuracy and validation accuracy }
    \caption{Convergence comparison within 100 iterations among our SPI-Optimizer, Momentum (MOM) \cite{rumelhart1986learning}, Gradient Descent (GD) \cite{cauchy1847methode}, Nesterov Accelerated Gradient (NAG)  \cite{nesterov1983method} and conditional integral (CI-$\beta$) on the quadratic function $f_5(\theta)$.}

% \ref{subfig:Nv1_weighted} to \ref{subfig:Nv6_weighted}

   \label{fig:cos}
\end{figure}



% \begin{figure}[htbp]
%     \centering
%     \newcommand{\colw}{0.48}
%     \newcommand{\figw}{1} % can bigger than 1
%     \begin{subfigure}[b]{0.8\linewidth}
%         \includegraphics[width=1.0\textwidth,clip]{{{sections/figures/figure_files/3_3_-2_1}}}
%         \captionsetup{labelformat=empty}
%          \caption{SPI}
%     \end{subfigure}%
    
%      % leave a blank line to change row       
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_0_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{MOM}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_1_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{GD}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_2_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{NAG}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_4_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{CI-β=0.1}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_5_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{CI-β=1}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_6_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{CI-β=10}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_7_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{CI-β=100}
%     \end{subfigure}
%     ~ 
%     \begin{subfigure}[b]{\colw\linewidth}
%         \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/3_8_-2_1}}}
%         \captionsetup{labelformat=empty}
%         \caption{CI-β=1000}
%     \end{subfigure}
% %    \caption{comparison of 4 popular methods on the MNIST dataset using CNN as the architecture for 20 epochs.Top row: the curves of training loss and validation loss.Bottom row: the curves of training accuracy and validation accuracy }
%     \caption{Comparison of SPI,CI with different T(threshold) and popular optimization methods (MOM,SGD,NAG) on the function $f(x,y)=-(cos(x)+1)*(cos(2y)+1)$. The optimals locates at the origin $(0, 0)$ (red circles). The initial point of the convergence process is $(-2, -1)$ (blue circles)}

% % \ref{subfig:Nv1_weighted} to \ref{subfig:Nv6_weighted}

%   \label{fig:cos}
% \end{figure}


==> sections/figures/trajectory_rosenbrock.tex <==

\begin{figure}[htbp]
    \centering
    % \newcommand{\colw}{0.48}
    % \newcommand{\figw}{1} % can bigger than 1
    \newcommand{\colw}{0.305}
    \newcommand{\figw}{1.0} % can bigger than 1
    \begin{subfigure}[b]{0.8\linewidth}
        \includegraphics[width=1.0\textwidth,clip]{{{sections/figures/figure_files/function_loss_curve5}}}
        \captionsetup{labelformat=empty}
        %\caption{\textbf{SPI}}
    \end{subfigure}%
    
    % leave a blank line to change row    
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_03}}}
        \captionsetup{labelformat=empty}
         \caption{\textbf{SPI}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_01}}}
        \captionsetup{labelformat=empty}
        \caption{GD}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_00}}}
        \captionsetup{labelformat=empty}
        \caption{MOM}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_02}}}
        \captionsetup{labelformat=empty}
        \caption{NAG}
    \end{subfigure}
    ~ 
    % \begin{subfigure}[b]{\colw\linewidth}
    %     \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_04}}}
    %     \captionsetup{labelformat=empty}
    %     \caption{CI-β=0.1}
    % \end{subfigure}
    % ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_05}}}
        \captionsetup{labelformat=empty}
        \caption{CI-β=1}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_06}}}
        \captionsetup{labelformat=empty}
        \caption{CI-β=10}
    \end{subfigure}
    % ~ 
    % \begin{subfigure}[b]{\colw\linewidth}
    %     \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_07}}}
    %     \captionsetup{labelformat=empty}
    %     \caption{CI-β=100}
    % \end{subfigure}
    % ~ 
    % \begin{subfigure}[b]{\colw\linewidth}
    %     \includegraphics[width=\figw\textwidth,clip]{{{sections/figures/figure_files/05_4_-1.5_08}}}
    %     \captionsetup{labelformat=empty}
    %     \caption{CI-β=1000}
    % \end{subfigure}
%    \caption{comparison of 4 popular methods on the MNIST dataset using CNN as the architecture for 20 epochs.Top row: the curves of training loss and validation loss.Bottom row: the curves of training accuracy and validation accuracy }
    \caption{Convergence comparison within 100 iterations among our SPI-Optimizer, Momentum (MOM) \cite{rumelhart1986learning}, Gradient Descent (GD) \cite{cauchy1847methode}, Nesterov Accelerated Gradient (NAG)  \cite{nesterov1983method} and conditional integral (CI-$\beta$) on the quadratic function $f_3(\theta)$.
        } 
   \label{fig:rosenbrock}
\end{figure}

==> sections/figures/windup.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{sections/figures/figure_files/windup} % don't need to specify .png or .jpg
\caption{integral windup}
\label{/fig:integral windup}
\end{figure}


==> sections/method_convergence_proof.tex <==
\subsection{Convergence of SPI-Optimizer}
\cite{richtarik2017stochastic}
\cite{loizou2017momentum}
Furthermore, we conduct theoretical analysis on the convergence of SPI-Optimizer, and show that under certain parameter settings(the value range of learning rate $r$ and momentum parameter $\alpha$) , 1) the convergence can be guaranteed, 2) the convergence rate is faster than SGD-MOM. More details about the proofs are presented in supplement. 
\begin{theorem}
Assume that the cost function $f(\theta)$ is a $\mu$-strongly convex and $L$-smooth function, and denote $\theta_{*}$ as the global minimum point satisfying $\nabla f(\theta_{*})=0$. For the SPI algorithm, as long as the value of $r$ and $\alpha$ is chosen in the range given below
\begin{gather*}
0<r<\frac{2\mu}{L^2},\ 0<\alpha<\frac{-p+\sqrt{p^2+16q}}{8}\\
p=4+4r+r L^2,\ q=2r\mu-r^2 L^2>0
\end{gather*}
SPI achieves the following guarantee, for all $k\geq 1$,
\begin{gather*}
\mathbf{E}\left\|\theta_k -\theta_* \right\|^2 \leq z^{k}(1+z-m) \mathbf{E}\left\|\theta_0 -\theta_* \right\|^2,\ z<1
\end{gather*}
where m,n and z are expressions of r and $\alpha$:
\begin{gather*}
m=1+3\alpha+2r\alpha+2\alpha^{2}+r\alpha L^2+r^2 L^2-2r\mu\\
n=\alpha+2r\alpha+2\alpha^{2},\ z=\frac{m+\sqrt{m^2+4n}}{2}<1
\end{gather*}
which means that $\mathbf{E}\left\|\theta_k -\theta_* \right\|^2$ converges to 0 exponentially.
\end{theorem}
The proof is given in the supplementary material.
%Our result indicates that as long as we choose the value of $r$ and $\alpha$ as requested, our SPI algorithm must converge in convex function situations. Additionally, we have used an inequality associated with our SPI algorithm in the proof, giving rise to the fact that the bound given by our method must be lower than that of SGD-MOM, which means as long as we choose parameters in the range given below, our method can converge faster than SGD-MOM.

==> sections/method_state_delay.tex <==

%\subsection{Re-examining PI Controller}
%
\textbf{State Delay: }
Recall that the objective of this feedback system is to let the gradient $\nabla L(\theta_{t+1})$ approach $\textbf{0}$, yet we only have the observation of the state $\nabla L(\tilde{\theta}_t)$.
This can be understood as a dynamic system with measurement latency or temporal delay. The larger the delay is, the more likely severe oscillation or unstable system occurs. 
Analogously, we define $d_{t+1} = \lvert\theta_{t+1} - \tilde{\theta}_t\rvert$ as \textit{state delay} in stochastic optimization:
\begin{equation} \label{eq:delay}
    \begin{aligned} 
    d_{t+1}^{GD}  &= |r \nabla L(\theta_t)| \\
    d_{t+1}^{MOM} &= |\alpha v_t + r \nabla L(\theta_t)| \\
    d_{t+1}^{NAG} &= |r \nabla L(\theta_t + \alpha v_t)|\\
    \end{aligned}
\end{equation}
%The ideal case of this dynamic system control would be that we can have the observation on the objective of the feedback system, i.e., we can predict the gradient of the future weight $\nabla L(\theta_\{t+1\})$.
%However, that is impossible. have In dynamic control applications, the different 

% One hypothesis is that for the same type of controller (say, PI controller) the optimizer with smaller state delay works better.
\textbf{Hypothesis}: One hypothesis is that for the momentum-based optimizer (PI controller), the optimizer with smaller state delay is highly likely having less oscillation, which is harmful for system stability.
% state delay <--> oscillation 
As the increase of $\alpha$ in Eqn. \ref{eq:delay} from GD to MOM, state delay of MOM $d_{t+1}^{\text{MOM}}$ has higher chance to be larger than that of GD $d_{t+1}^{\text{GD}}$, which explains why MOM usually oscillates more during optimization process.
% \Ji{The convergence path on the banana function don't have much oscillation --> MOM works the best. For the quadratic function, oscillation appears --> NAG works better than MOM. GD doesn't oscillate much but convergant slowly}
Similarly, NAG can be understood as a more robust PI controller with smaller state delay under the assumption that both $\nabla L(\theta_t + \alpha v_t)$ and $\nabla L(\theta_t)$ share the same probabilistic distribution.
Some experiments shown in the next section intuitively validates this hypothesis. 

The key idea of SPI is that when the oscillation is detected we reduce the state delay by assigning $d_{t+1}^{\text{SPI}} = d_{t+1}^{\text{GD}}$, otherwise, keep using the PI controller to speed up.

==> sections/tables/c100_alexnet.tex <==
\begin{table}[htbp]
\centering
\small
%\hspace{-0.5cm}
\begin{tabular}{cccccccccc}
Optimization Methods  & \begin{tabular}{@{}c@{}}lr=0.05 \\ \end{tabular}
        & \begin{tabular}{@{}c@{}}lr=0.1 \\\end{tabular}
        & \begin{tabular}{@{}c@{}}lr=0.18 \\ \end{tabular} \\
    \hline
    MOM &59.158\%         &68.312\%	&-    \\
    \hline
    SGD &60.089\%	       &60.240\%	        &60.079\%\\
    \hline
    NAG &58.945\%	       &67.091\%	        &-\\
     \hline
    SPI &\textbf{58.188\%}          &\textbf{57.179\%}   &\textbf{57.223\%}\\
    \hline    
\end{tabular}
%\hspace{0.3cm}
% put caption below the \end{tabular} to put the caption at the bottom
\captionof{table}{
Final test errors achieved by SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) with different learning rate using AlexNet on CIFAR-100 for 50 epoches.\wang{The symbol $-$ represents that the algorithm does not converge under the learning rate}
} \label{tab:c100_alexnet}
\end{table}
% \hline
% IS-T=0.1 \\ $\beta=6$ $\gamma=80\%$ \\ w/o weighted average &  0.448 &   0.251 &       0.798 & 0.228 \\

==> sections/tables/mnist_cnn.tex <==
\begin{table}[htbp]
\centering
\small
%\hspace{-5cm}
\begin{tabular}{cccccccccc}
Optimization Methods   & \begin{tabular}{@{}c@{}}lr=0.08 \\ \end{tabular}
        & \begin{tabular}{@{}c@{}}lr=0.12 \\\end{tabular}
        & \begin{tabular}{@{}c@{}}lr=0.15 \\\end{tabular}
        & \begin{tabular}{@{}c@{}}lr=0.2 \\ \end{tabular} \\
    \hline
    MOM &1.734\%	        &1.720\%\%	&1.933\% &NaN\\
    \hline
    SGD      &1.167\%	        &1.111\%	            &1.134\%  &4.847\\ 
    \hline
    NAG      &1.338\%          &1.772\%	            &2.527\%  &NaN\\
     \hline
    SPI &\textbf{1.101\%}        &\textbf{1.070\%}              &\textbf{1.122\%} &\textbf{1.510}\\
    \hline    
\end{tabular}
%\hspace{0.3cm}
% put caption below the \end{tabular} to put the caption at the bottom
\captionof{table}{Final test errors achieved by SPI-Optimizer and popular optimization methods(MOM, SGD, NAG) with different learning rate using CNN on MNIST.} \label{tab:mnist_cnn}
\end{table}
% \hline
% IS-T=0.1 \\ $\beta=6$ $\gamma=80\%$ \\ w/o weighted average &  0.448 &   0.251 &       0.798 & 0.228 \\

==> sections/tables/networks.tex <==

\begin{table*}[tb]
\centering
\small
%\hspace{-0.5cm}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Optimization Methods  & \begin{tabular}{@{}c@{}}Depth-k \\ \end{tabular}
        & \begin{tabular}{@{}c@{}}Params \\\end{tabular}
                & \begin{tabular}{@{}c@{}}C10(original) \\\end{tabular}
        & \begin{tabular}{@{}c@{}}C10(SPI) \\\end{tabular}
                & \begin{tabular}{@{}c@{}}C100(original) \\\end{tabular}
        & \begin{tabular}{@{}c@{}}C100(SPI) \\\end{tabular}\\
      %  & \begin{tabular}{@{}c@{}}Epoches \\ \end{tabular} \\
    \hline
%    MOM &0.574	&0.284    &\textbf{0.627}	 \\
 %   \hline
 %   SGD      &      0.448	&\textbf{0.234}	&0.706	\\
   \hline
    CliqueNet\cite{}&36-12     &   0.94M\%	&5.93\%&\textbf{	5.75}\%&27.32\%&\textbf{XX\% }	\\
     \hline
    CliqueNet \cite{}&80-18   &   10.14M\%	&5.06\%&\textbf{4.10}\% &23.14\%&\textbf{XX\%}	\\
    \hline
    WRN\cite{}&11M\%&16-8	&4.81\%	&4.32\%&  22.07\%	&\textbf{20.89}\%\\
    \hline
    WRN \cite{}&28-10&36.5M\%	&4.17\%	&3.86\%&  20.50\%	&\textbf{19.23}\%\\
    \hline
    Resnet110\cite{}&110 &1.7M\%	&6.43\%	&xx\%&   25.16\%	&\textbf{xxxx}\%\\
    \hline    

 
\end{tabular}
%\hspace{0.3cm}
% put caption below the \end{tabular} to put the caption at the bottom
\captionof{table}{
Test error of the state-of-the-art network on CIFAR-10 and CIFAR-100.}
\label{tab:generalization}
\end{table*}
% \hline
% IS-T=0.1 \\ $\beta=6$ $\gamma=80\%$ \\ w/o weighted average &  0.448 &   0.251 &       0.798 & 0.228 \\
